SPARTan: Scalable PARAFAC2 for Large & Sparse Data

In exploratory tensor mining, a common problem is how to analyze a set of variables across a set of subjects whose observations do not align naturally. For example, when modeling medical features across a set of patients, the number and duration of treatments may vary widely in time, meaning there is no meaningful way to align their clinical records across time points for analysis purposes. To handle such data, the state-of-the-art tensor model is the so-called PARAFAC2, which yields interpretable and robust output and can naturally handle sparse data. However, its main limitation up to now has been the lack of efficient algorithms that can handle large-scale datasets. In this work, we fill this gap by developing a scalable method to compute the PARAFAC2 decomposition of large and sparse datasets, called SPARTan. Our method exploits special structure within PARAFAC2, leading to a novel algorithmic reformulation that is both fast (in absolute time) and more memory-efficient than prior work. We evaluate SPARTan on both synthetic and real datasets, showing 22X performance gains over the best previous implementation and also handling larger problem instances for which the baseline fails. Furthermore, we are able to apply SPARTan to the mining of temporally-evolving phenotypes on data taken from real and medically complex pediatric patients. The clinical meaningfulness of the phenotypes identified in this process, as well as their temporal evolution over time for several patients, have been endorsed by clinical experts.

==> content/abstract.tex <==
\begin{abstract}
The canonical polyadic (CP) decomposition is considered as the most practical approach for exploratory tensor mining. In part, this is due to its intuitive output structure and its uniqueness properties, as both boost intepretability. Another reason is the development of efficient algorithms and software for sparse CP decompositions, enabling a wide variety of data mining applications.

However, CP cannot support the following general framework: we observe a set of variables across a set of subjects, where the various observations do not exhibit a natural alignment among the subjects. For example, this use case arises when modeling the medical features across a set of patients, over the course of their---varying in length and lacking a meaningful alignment---clinical records over time. A more flexible version of CP, the PARAFAC2 decomposition, can naturally frame this type of problems. At the same time, PARAFAC2 preserves the desirable properties of CP, such as uniqueness. Its main limitation up to now though  has been the lack of efficient algorithms being able to tackle large-scale data.

In this work, we fill this gap, by proposing a scalable method for PARAFAC2 decomposition of large and sparse datasets, called \mname. Through scaling up the core computational kernel arising in the PARAFAC2 fitting algorithm, \mname achieves the best of both worlds in terms of speed and memory efficiency. As we evaluated on multiple real and synthetic datasets, \mname is both faster than the baseline achieving up to $22\times$ performance gain, and it is also more scalable, by enabling PARAFAC2 execution for larger problem instances for which the baseline fails. We demonstrate the application of our approach on mining temporally-evolving phenotypes on real medically complex pediatric patients. The clinical meaningfulness of the phenotypes identified as well as their temporal evolution over time for several patients were endorsed by clinical experts.%confirming the interpretability and usefulness of the proposed approach.
\end{abstract}


==> content/intro-orig.tex <==
\section{Introduction}\label{sec:intro}

% \begin{figure}
% \centering
% \includegraphics[width=0.3\textwidth]{results/synthetic_rank10}
% \caption{\footnotesize Synthetic Data ($R=10$): We construct increasingly denser datasets. For half a billion non-zeros, \mname runs one iteration in $15$ minutes, while the baseline approach takes $200$ minutes for the same computation. %Time is averaged over $10$ iterations.
% %this figure can probably be moved to intro,change \# in x-asis to something more easily understandable like 500K to 500M? 
% %\jsedit{can we show one that is beyond 1 billion?}
% }
% \label{fig:synthetic_rank10}
% \end{figure}

\begin{table*}
\centering
\small
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|}
\hline
\textbf{Target Rank} & \multicolumn{5}{c||}{\textbf{10}} & \multicolumn{5}{c|}{\textbf{40}} \\ \hline
\textbf{\#nnz(Millions)} & \textbf{63} & \textbf{125} & \textbf{250} & \textbf{500} & \textbf{750}& \textbf{63} & \textbf{125} & \textbf{250} & \textbf{500} & \textbf{750} \\
\hline
\mname & 7.4 & 8.9 & 11.5 & 15.4 & 33.7 & 14 & 18.4 & 61 & 114 & 123.5 \\
\hline
Sparse PARAFAC2 & 24.4 & 60.1 & 72.3 & 194.5 & \textbf{\color{red}OoM} & 275.2 & 408.1 & \textbf{\color{red}OoM} & \textbf{\color{red}OoM} & \textbf{\color{red}OoM} \\
\hline
\end{tabular}
\caption{\footnotesize Running time comparison: Time in minutes of one iteration for increasingly larger datasets (63m to 750m) and fixed target rank (two cases considered: $R=\{10, 40\}$). The mode sizes for the datasets constructed are: $1$Mil.~subjects, $5$K variables and $100$ observations per subject. \textbf{\color{red}OoM} (Out of Memory) denotes that the execution failed due to the excessive amount of memory requested. Experiments are conducted on a server with 1TB of RAM.}
\label{table:synthetic}
\end{table*}

Due to their capability of naturally expressing multi-modal data, \textit{tensors} are very popular in data mining. The canonical polyadic (CP) decomposition (also known as PARAFAC or CANDECOMP)~\cite{hitchcock1927expression,harshman1970foundations,carroll1970analysis} is one of the most popular tensor analysis methods. In part, this happens because of the CP model's \textit{intuitive output structure} as a sum of multi-way outer products:~$\T{X}~\approx~\sum_{r=1}^R \V{u}_r \circ \V{v}_r \circ \V{w}_r$, where $\V{u}_r, \V{v}_r, \V{w}_r $ are column vectors of size $I, J, K$ respectively for an input tensor $\T{X}$ of size $I~\times~J~\times~K$. Through this formulation, each rank-one component serves as a latent data concept. Another important property of CP is \textit{uniqueness}, under very mild conditions, up to scaling and permutation of the $R$ components~\cite{kruskal1977three,sidiropoulos2000uniqueness}. In exploratory data analysis, uniqueness is imperative towards reliable model interpretation: it guarantees that the latent factors pursued are the actual ones, rather than an arbitrarily rotated version of them~\cite{kolda2009tensor,papalexakis2016tensors,sidiropoulos2016tensor}. Finally, efficient sparse CP algorithms~\cite{bader2007efficient,chi2012tensors} and implementation~\cite{TTB_Software} do exist, which enabled important real-world applications (e.g., healthcare~\cite{ho2014limestone,ho2014marble}, social networks~\cite{dunlavy2011temporal,papalexakis2015p}) %as tensors are mostly \textit{sparse} in those data mining applications. 

%\jsedit{add all the appropriate citations here. I remove a few paragraphs about CP to get to the main message quickly} \jsedit{We should show the formal math definition of CP here. I don't think we need to hold off the exact definition.}
%\reminder{V: High-level comment: We are using lack of uniqueuness as a strong counter-argument for previous works. We know what uniqueness is and why it's necessary, but I don't think it shows in the intro. Maybe a couple of sentences exaplaining why the rotations in a non-unique model can have bad consequences in interpretation. Maybe a couple of sentences in the intro and a more extended paragraph somewhere in the text (and refer to that paragraph in the intro) Otherwise a reader might say "well I don't really care about this uniqueness thing so far, why should I care now??"}

%Non-unique models result in several mathematically equivalent (arbitrarily rotated) solutions; this is problematic, since only one of those solutions is describing the true underlying latent information. This is uncovered by CP, as guaranteed by the uniqueness property~\cite{papalexakis2016tensors}. 

%Thanks to the simple output structure and uniqueness property \jsedit{Do we want to say anything about efficient CP method for sparse data? I think that is another reason why CP is popular for data analysis}, CP is considered as the standard tool for \textit{exploratory} tensor analysis, where users will try to interpret the output of a tensor decomposition for knowledge discovery. As a result, CP has attracted a lot of attention from various research fields, such as Chemometrics~\cite{bro1997parafac} and Signal Processing~\cite{sidiropoulos2016tensor} (cite also Cichocki?), where data are mostly arising as dense tensors. 


Despite its advantages, CP expects the input tensor in a regular \enquote{cube} shape, assuming all the elements are comparable along each mode~\footnote{This holds for other variants of CP as well~\cite{harshman2003shifted,morup2008shift,morup2011modeling}.}. %This is a common assumption also made by other widely-used tensor models in data mining, such as Tucker~\cite{tucker1966some}.
However, there are cases when a tensor is \enquote{irregular}, in the sense that it consists of a collection of matrices, %\jsedit{can we say a collection of tensors instead to be more general or we only can handle matrices?}
having a non-comparable mode with potentially varying sizes across them. %A typical example of that arises when trying to model the {\it time} mode.

\noindent{\bf Motivating Scenario:} Electronic Health Records (EHRs) are broadly deployed across clinics and hospitals in the US to capture longitudinal patient information. Given a patient, her EHR can be represented as an event sequence of multiple modalities including diagnoses, medications, procedures, and lab results. An important characteristic of such event sequences is that there is no simple time alignment across patients. 
%For example, consider that two patients visited the hospital on Jan 1st, where patient $A$ visited for the first time and was diagnosed with disease $X$, while patient $B$ had disease $X$ diagnosed a long time ago and had severe complications with $X$ on that day. Clearly, it is not sensible to directly compare those two patients based on their data from Jan 1st. Moreover these two patients may have very different length of visit history as $B$ can have much longer medical history than $A$.
First, different patients exhibit varying lengths of records between the first admission and the most recent hospital discharge. %In addition, even if the lengths of patients' records are exactly the same, 
Additionally, even if the patient records' length is the same, it is not sensible to align them chronologically as disease stages and patient progress vary. %Any alignment attempt would assume the same  only capture common medical concepts among patients occurring the exact same date. Clearly, this is not the desired approach. 
Instead, our ultimate goal should be to capture the flexible evolution patterns of clinical concepts over time for patients with: \textit{a)} varying lengths of medical history and \textit{b)} variations on the exact time that those trends are expressed within the medical history.

In general, it is extremely challenging to perform multi-modal analysis including the \enquote{non-matching} time mode, without resorting to some form of preprocessing. One standard form of preprocessing pertains to collapsing the time mode with simple aggregated statistics such as sum or average.
This methodology has been widely employed for healthcare applications, where there have been sophisticated tensor methods based on the CP model, such as in~\cite{ho2014limestone,ho2014marble,wang2015rubik}. Those methods essentially ignore the time mode, by accumulating counts for each event, as a preprocessing step. Inevitably, they fall short of modeling the intricate temporal patterns in the data. Another preprocessing methodology is the creation of more sophisticated temporal features, such as the Wavelet transform used in ~\cite{sun2008two}. However, this direction assumes that the temporal measures are continuous and sufficiently long, which is not the case in many data mining applications, as in the EHR example above.

   %\jsedit{we should also mention and cite those 2-step processes to extract more sophisticated temporal features such as performing Wavelet transform (my PKDD paper a while ago), and I think Evrim Acar on EEG data and Rasmus probably have something as well on food measurements. But the key distinction is that they assume continuous and comparable temporal measures, which are not available in many data mining applications}

%One could try to perform zero-padding of the time mode, based on the patient with the largest number of visits. Such an approach though implies that patient histories and clinical events follow a global alignment, which is definitely not the case. Another approach would be to vertically concatenate the EHRs and attempt to factorize the resulting matrix; in that case though, the interpretation of the individual patient visits is unclear since they have been mixed to form a large all\_visits-by-variables matrix.

Specifically for healthcare applications, there are proposed methodologies such as in~\cite{zhou2014micro,wang2013framework,wang2014densitytransfer}, which do model the temporal evolution of clinical concepts for each patient, but they all lack of the \textit{uniqueness} property in their models. Thus, it becomes harder to reliably extract the actual latent concepts as an equivalent arbitrary rotation of them will provide the same fit.

\begin{figure}
\centering
\includegraphics[scale=0.15]{figures/parafac2}
\caption{\footnotesize Illustration of the PARAFAC2 model.}
\label{fig:parafac2}
\end{figure}

In fact, the type of data in the motivating example are quite general: %\enquote{multiset} data(cite). \jsedit{What are the related work in modeling multiset data? Why don't we compare with them? How about joint matrix factorization?}
consider that we have $K$ subjects, for which we record $J$ variables and we permit each $k$-th subject to have $I_k$ observations, which are not necessarily comparable among the different subjects. The input expected by the PARAFAC2 model, first introduced by Harshman~\cite{Hars1972b}, is a perfect match for this type of data. It can be considered as a more flexible version of the CP: while CP applies the
same factors across a collection of matrices, PARAFAC2 instead applies the same
factor along one mode and allows the other factor matrix to vary~\cite{kolda2009tensor}.  %, by relaxing a few constraints %\reminder{V: maybe one sentence explaining why or what constraints?}. 
At the same time, it preserves the desirable properties of CP, such as uniqueness~\cite{harshman1996uniqueness,ten1996some,kiers1999parafac2,stegeman2015multi}. As shown in Figure~\ref{fig:parafac2}, PARAFAC2 approximates each one of the input matrices as: $\M{X}_k \approx \M{U}_k ~ \M{S}_k ~ \M{V}^T$, where $\M{U}_k$ is of size $I_k \times R$, $I_k$ is the number of observations available for the $k$-th subject and $R$ the target rank of the decomposition.  %We will expand on the equivalence of the factors $\{\M{S}_k\}, \M{V}$ with the ones of the CP model, as well as on the necessary details of PARAFAC2 in Section~\ref{sec:sparafac2}. %Instead of constraining all $\M{U}_k$ matrices to be the equal (as in classical CP), PARAFAC2 enforces that the cross-product $\M{U}_k^T \M{U}_k$ is constant over $k$ (over all subjects). The rest of the model's factors are direct analogues of the CP factor matrices. We will expand on the model's details in Section~\ref{sec:back}.
%\jsedit{Can we just move the parafac2 mathematic definition here? I find it more difficult to read this long description than just showing the math}


%Probably because of the lack of efficient sparse algorithms, PARAFAC2 has not been utilized widely in data mining. \kimis{Awesome point! Bro makes exactly this point in his PARAFAC tutorial~\cite{bro1997parafac} for PARAFAC2: \enquote{The PARAFAC2 model has not yet been used very extensively maybe because the implementations so far have been complicated and slow.}} 

% The lack of efficient algorithms for PARAFAC2 decomposition has been highlighted as a major challenge by Rasmus Bro~\cite{bro1997parafac}:
% \begin{quote}
% \textit{The PARAFAC2 model has not yet been used very extensively maybe because the implementations so far have been complicated and slow.}
% \end{quote}

The lack of efficient PARAFAC2 decomposition algorithms has been underlined in the literature as a reason for its limited popularity~\cite{bro1997parafac,chew2007cross}. Overall, PARAFAC2 has been mostly used for dense data (e.g.,~\cite{kiers1999parafac2}) or sparse data with a small number of subjects involved \cite{chew2007cross}. To the best of our knowledge, no work has assessed PARAFAC2 for large-scale sparse data, as well as the challenges arising by doing so. 

In this paper, we propose \mname (abbreviated from Scalable PARafac Two) for large and sparse datasets. Our main methodological advancement is a new algorithm for scaling up the core computational kernel arising in the PARAFAC2 fitting algorithm.
\mname achieves the best of both worlds in terms of speed and memory efficiency: \textit{a)} it is \textit{faster} than a highly-optimized baseline in all cases considered for both real (Tables~\ref{table:choa_scale_rank},\ref{table:movielens_scale_rank},\ref{table:choa_scale_fixed_rank},\ref{table:movielens_scale_fixed_rank}) and synthetic (Table~\ref{table:synthetic}) datasets, achieving up to %over an order of magnitude
$22\times$ performance gain; \textit{b)} at the same time, \mname is \textit{more scalable}, in that it can execute in reasonable time for large problem instances when the baseline fails due to excessive memory consumption (Table~\ref{table:synthetic}).

We summarize our contributions as:
\begin{itemize}[leftmargin=5.5mm]
\item \textbf{Scalable PARAFAC2 method:} We propose a scalable algorithm fitting the PARAFAC2 model on large and sparse data.
\item \textbf{Evaluation on various datasets:} We evaluate the scalability of our approach using datasets originating from two different application domains, namely longitudinal EHR and time-evolving movie ratings' data. Additionally, we perform synthetic data experiments.
\item \textbf{Real-world case study}: We performed a case study of applying \mname on
temporal phenotyping over medically complex pediatric patients in collaboration with Children's Healthcare of Atlanta (CHOA). The phenotypes and temporal trends discovered were endorsed by a clinical expert from CHOA. %\reminder{We may need a word slightly more memorable and strong than ``confirmed'' here. Also, if we have any number on what percentage of the results the expert found to be good, here is a good place to mention that (and maybe the abstract too)}
\end{itemize}
To promote reproducibility, our code will be open-sourced. For reviewing purposes, it can downloaded from (\kimis{Todo: Polish code and provide dropbox link}).

==> results/table2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \scriptsize
    \begin{tabular}{lr}
    \textbf{Old Classics} & \multicolumn{1}{l}{\textbf{Weight}} \\
    Casablanca (1942),Drama|Romance & 0.1 \\
    Citizen Kane (1941),Drama|Mystery & 0.1 \\
    Chinatown (1974),Crime|Film-Noir|Mystery|Thriller & 0.1 \\
    Rear Window (1954),Mystery|Thriller & 0.1 \\
    Annie Hall (1977),Comedy|Romance & 0.1 \\
    North by Northwest (1959),Action|Adventure|Mystery|Romance|Thriller & 0.1 \\
    Graduate, The (1967),Comedy|Drama|Romance & 0.09 \\
    Dr. Strangelove or: How I Learned to Stop Worrying and Love the Bomb (1964),Comedy|War & 0.09 \\
    Vertigo (1958),Drama|Mystery|Romance|Thriller & 0.09 \\
    Godfather, The (1972),Crime|Drama & 0.09 \\
    \textbf{Action Movies} & \multicolumn{1}{l}{\textbf{Weight}} \\
    Total Recall (1990),Action|Adventure|Sci-Fi|Thriller & 0.1 \\
    Predator (1987),Action|Sci-Fi|Thriller & 0.09 \\
    RoboCop (1987),Action|Crime|Drama|Sci-Fi|Thriller & 0.09 \\
    Lethal Weapon (1987),Action|Comedy|Crime|Drama & 0.09 \\
    Starship Troopers (1997),Action|Sci-Fi & 0.09 \\
    Die Hard 2 (1990),Action|Adventure|Thriller & 0.08 \\
    Aliens (1986),Action|Adventure|Horror|Sci-Fi & 0.08 \\
    Abyss, The (1989),Action|Adventure|Sci-Fi|Thriller & 0.08 \\
    Terminator, The (1984),Action|Sci-Fi|Thriller & 0.08 \\
    Die Hard (1988),Action|Crime|Thriller & 0.08 \\
    \textbf{Romance/Comedy Movies} & \multicolumn{1}{l}{\textbf{Weight}} \\
    Erin Brockovich (2000),Drama & 0.09 \\
    Wedding Singer, The (1998),Comedy|Romance & 0.08 \\
    Shrek (2001),Adventure|Animation|Children|Comedy|Fantasy|Romance & 0.08 \\
    Good Will Hunting (1997),Drama|Romance & 0.08 \\
    Ferris Bueller's Day Off (1986),Comedy & 0.08 \\
    Bridget Jones's Diary (2001),Comedy|Drama|Romance & 0.08 \\
    Little Mermaid, The (1989),Animation|Children|Comedy|Musical|Romance & 0.08 \\
    Meet the Parents (2000),Comedy & 0.08 \\
    Notting Hill (1999),Comedy|Romance & 0.08 \\
    As Good as It Gets (1997),Comedy|Drama|Romance & 0.08 \\
    \end{tabular}%
  \caption{\footnotesize MovieLens dataset: Movie groupings \kimis{Will probably be omitted from the submission.}}
  \label{tab:mv_clusters}
\end{table}%

